ORACLE: Occlusion-Resilient and Self-Calibrating mmWave Radar Network for People Tracking

Millimeter wave (mmWave) radar sensors are emerging as valid alternatives to cameras for the pervasive contactless monitoring of people in indoor spaces. However, commercial mmWave radars feature a limited range (up to $6$-$8$ m) and are subject to occlusion, which may constitute a significant drawback in large, crowded rooms characterized by a challenging multipath environment. Thus, covering large indoor spaces requires multiple radars with known relative position and orientation and algorithms to combine their outputs. In this work, we present ORACLE, an autonomous system that (i) integrates automatic relative position and orientation estimation from multiple radar devices by exploiting the trajectories of people moving freely in the radars' common fields of view, and (ii) fuses the tracking information from multiple radars to obtain a unified tracking among all sensors. Our implementation and experimental evaluation of ORACLE results in median errors of $0.12$ m and $0.03^\circ$ for radars location and orientation estimates, respectively. Fused tracking improves the mean target tracking accuracy by $27\%$, and the mean tracking error is $23$ cm in the most challenging case of $3$ moving targets. Finally, ORACLE does not show significant performance reduction when the fusion rate is reduced to up to 1/5 of the frame rate of the single radar sensors, thus being amenable to a lightweight implementation on a resource-constrained fusion center.

==> biblio-backup.tex <==
@article{savazzi2019use,
  title={{On the use of stray wireless signals for sensing: A look beyond 5G for the next generation of industry}},
  author={Savazzi, Stefano and others},
  journal={Computer},
  volume={52},
  NOnumber={7},
  NOpages={25--36},
  month={Jun},
  year={2019},
  publisher={IEEE}
}

@article{guo2020deepstore,
  title={Deepstore: understanding customer behaviors in unmanned stores},
  author={Guo, Bin and others},
  journal={IT Professional},
  volume={22},
  NOnumber={3},
  NOpages={55--63},
  month={May},
  year={2020},
  publisher={IEEE}
}


@article{hassan2017application,
  title={{Application of wireless technology for control: A WirelessHART perspective}},
  author={Hassan, Sabo Miya and others},
  journal={Procedia Computer Science},
  volume={105},
  NOpages={240--247},
  month={Dec},
  year={2017},
  publisher={Elsevier}
}


@article{shah2019rf,
  title={{RF sensing technologies for assisted daily living in healthcare: A comprehensive review}},
  author={Shah, Syed Aziz and Fioranelli, Francesco},
  journal=IEEE_M_AES,
  NOvolume={34},
  NOnumber={11},
  NOpages={26--44},
  month={Nov},
  year={2019},
  publisher={IEEE}
}

@article{vandersmissen2018indoor,
  title={{Indoor person identification using a low-power FMCW radar}},
  author={Vandersmissen, Baptist and Knudde, Nicolas and Jalalvand, Azarakhsh and Couckuyt, Ivo and Bourdoux, Andr{\'e} and De Neve, Wesley and Dhaene, Tom},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={56},
  NOnumber={7},
  NOpages={3941--3952},
  month={Jul},
  year={2018},
  publisher={IEEE}
}

@inproceedings{jin2019multiple,
	title={{Multiple patients behavior detection in real-time using mmwave radar and deep CNNs}},
	author={Jin, Feng and others},
	booktitle={IEEE Radar Conference (RadarConf)},
	NONOaddress={Boston, Massachusetts, USA},
	month={Apr},
	year={2019},
	organization={IEEE}
}

@inproceedings{singh2019radhar,
  title={{Radhar: Human activity recognition from point clouds generated through a millimeter-wave radar}},
  author={Singh, Akash Deep and others},
  booktitle={Proc.~ACM mmNets},
  NOpages={51--56},
  year={2019}
}

@article{cao2018radar,
  title={{Radar-ID: human identification based on radar micro-Doppler signatures using deep convolutional neural networks}},
  author={Cao, Peibei and Xia, Weijie and Ye, Ming and Zhang, Jutong and Zhou, Jianjiang},
  journal={{IET} Radar, Sonar \& Navigation},
  volume={12},
  NOnumber={7},
  NOpages={729--734},
  month={Jul},
  year={2018},
  publisher={IET}
}

@inproceedings{knudde2017indoor,
	title={{Indoor tracking of multiple persons with a 77 GHz MIMO FMCW radar}},
	author={Knudde, Nicolas and others },
	booktitle={Proc.~EURAD},
	NOaddress={Nuremberg, Germany},
	month={Oct},
	year={2017},
}

@inproceedings{lu2020see,
	title={{See Through Smoke: Robust Indoor Mapping with Low-cost mmWave Radar}},
	author={Lu, Chris Xiaoxuan and Rosa, Stefano and Zhao, Peijun and Wang, Bing and Chen, Changhao and Stankovic, John A and Trigoni, Niki and Markham, Andrew},
	booktitle={18th International Conference on Mobile Systems, Applications, and Services (MobiSys)},
	NONOaddress={Toronto, Canada},
	month={Jun},
	year={2020}
}

@article{seifert2019toward,
	title={{Toward unobtrusive in-home gait analysis based on radar micro-Doppler signatures}},
	author={Seifert, Ann-Kathrin and Amin, Moeness G and Zoubir, Abdelhak M},
	journal={IEEE Transactions on Biomedical Engineering},
	volume={66},
	NOnumber={9},
	NOpages={2629--2640},
	month={Jan},
	year={2019},
	publisher={IEEE}
}


@article{chen2018personnel,
  title={{Personnel recognition and gait classification based on multistatic micro-Doppler signatures using deep convolutional neural networks}},
  author={Chen, Zhaoxi and Li, Gang and Fioranelli, Francesco and Griffiths, Hugh},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={15},
  NOnumber={5},
  NOpages={669--673},
  month={May},
  year={2018}
}

@inproceedings{jalalvand2019radar,
  title={{Radar signal processing for human identification by means of reservoir computing networks}},
  author={Jalalvand, Azarakhsh and Vandersmissen, Baptist and De Neve, Wesley and Mannens, Erik},
  booktitle={{IEEE Radar Conference (RadarConf)}},
  NONOaddress={Boston, Massachusetts USA},
  month={Apr},
  year={2019}
}


@inproceedings{polfliet2018structured,
  title={{Structured inference networks using high-dimensional sensors for surveillance purposes}},
  author={Polfliet, Vincent and Knudde, Nicolas and Vandersmissen, Baptist and Couckuyt, Ivo and Dhaene, Tom},
  booktitle={International Conference on Engineering Applications of Neural Networks (EANN)},
NONOaddress={Crete, Greece},
month={May},
  year={2018},
}

@inproceedings{abdulatif2019person,
title={{Person identification and body mass index: A deep learning-based study on micro-Dopplers}},
author={Abdulatif, Sherif  and  Aziz, Fady and Armanious, Karim  and  Kleiner, Bernhard and Yang, Bin and Schneider, Urs},
booktitle={{IEEE} Radar Conference (RadarConf)},
  NONOaddress={Boston, Massachusetts USA},
  month={Apr},
year={2019}
}

@inproceedings{zhao2019mid,
  title={{mID: Tracking and Identifying People with Millimeter Wave Radar}},
  author={Zhao, Peijun and others},
  booktitle={{Proc.~DCOSS}},
NOaddress={Santorini Island, Greece},
month={May},
  year={2019},
}


@article{yang2019person,
  title={{Person Identification Using Micro-Doppler Signatures of Human Motions and UWB Radar}},
  author={Yang, Yang and Hou, Chunping and Lang, Yue and Yue, Guanghui and He, Yuan and Xiang, Wei},
  journal={IEEE Microwave and Wireless Components Letters},
  volume={29},
  NOnumber={5},
  NOpages={366--368},
  month={May},
  year={2019}
}

@inproceedings{trommel2016multi,
  title={{Multi-target human gait classification using deep convolutional neural networks on micro-Doppler spectrograms}},
  author={Trommel, RP and Harmanny, RIA and Cifola, L and Driessen, JN},
  booktitle={European Radar Conference (EuRAD)},
  NONOaddress={London, United Kingdom},
  month={Oct},
  year={2016}
}

@inproceedings{weishaupt2018vital,
  title={{Vital Sign Localization and Measurement Using an LFMCW MIMO Radar}},
  author={Weishaupt, Fabio and Walterscheid, Ingo and Biallawons, Oliver and Klare, Jens},
  booktitle={19th International Radar Symposium (IRS)},
  NONOaddress={Bonn, Germany},
  month={Jun},
  year={2018}
}

@article{hsieh2015uwb,
  title={{A UWB radar signal processing platform for real-time human respiratory feature extraction based on four-segment linear waveform model}},
  author={Hsieh, Chi-Hsuan and Chiu, Yu-Fang and Shen, Yi-Hsiang and Chu, Ta-Shun and Huang, Yuan-Hao},
  journal={IEEE transactions on biomedical circuits and systems},
  volume={10},
  NOnumber={1},
  NOpages={219--230},
  month={Feb},
  year={2015}
}

@inproceedings{tahmoush2009radar,
  title={{Radar micro-Doppler for long range front-view gait recognition}},
  author={Tahmoush, Dave and Silvious, Jerry},
  booktitle={IEEE 3rd International Conference on Biometrics: Theory, Applications, and Systems},
  NONOaddress={Washington DC, Columbia, USA},
  month={Sep},
  year={2009}
}

@article{kalman1960new,
  title={{A new approach to linear filtering and prediction problems}},
  author={Kalman, Rudolf Emil},
  journal={ASME Trans., J Basic Eng},
  NOvolume={82, (Series D)},
  NOnumber={1},
  NOpages={35--45},
  year={1960},
  publisher={ASME}
}

@article{wagner2017radar,
  title={{Radar signal processing for jointly estimating tracks and micro-Doppler signatures}},
  author={Wagner, Thomas and others},
  journal={IEEE Access},
  volume={5},
  NOpages={1220--1238},
month={Feb},
  year={2017},
  publisher={IEEE}
}

@inproceedings{ester1996density,
  title={{A density-based algorithm for discovering clusters in large spatial databases with noise}},
  author={Ester, Martin and others},
  booktitle={Proc.~ACM KDD},
  NONOaddress={Portland, Oregon, USA},
  month={Aug},
  year={1996}
}

@article{patole2017automotive,
  title={{Automotive radars: A review of signal processing techniques}},
  author={Patole, Sujeet Milind and others},
  journal=IEEE_M_SP,
  NOvolume={34},
  NOnumber={2},
  NOpages={22--35},
  month={Mar},
  year={2017}
}

@article{chen2006micro,
  title={{Micro-Doppler effect in radar: phenomenon, model, and simulation study}},
  author={Chen, Victor and Li, Fayin and Ho, S and Wechsler, Harry},
  journal=IEEE_J_AES,
  volume={42},
  NOnumber={1},
  NOpages={2--21},
  month={Aug},
  year={2006}
}

@inproceedings{chen2000analysis,
  title={{Analysis of radar micro-Doppler with time-frequency transform}},
  author={Chen, Victor},
  booktitle={Proceedings of the Tenth IEEE Workshop on Statistical Signal and Array Processing},
  NONOaddress={Pocono Manor, Pennsylvania, USA},
  month={Aug},
  year={2000}
}

@inproceedings{winkler2007range,
  title={{Range Doppler detection for automotive FMCW radars}},
  author={Winkler, Volker},
  booktitle={European Radar Conference (EuRAD)},
  NONOaddress={Munich, Germany},
  month={Oct},
  year={2007}
}

@article{bar2009probabilistic,
  title={{The probabilistic data association filter}},
  author={Bar-Shalom, Yaakov and Daum, Fred and Huang, Jim},
  journal={IEEE Control Syst. Mag.},
  volume={29},
  NOnumber={6},
  NOpages={82--100},
  month={Dec},
  year={2009},
}

@inproceedings{franken2017range,
  title={{Range/Doppler tracking with the Kalman filter and its relatives—A comparative study}},
  author={Fr{\"a}nken, Dietrich and Woischneck, Sebastian},
  booktitle={{Sensor Data Fusion: Trends, Solutions, Applications (SDF)}},
  NOpages={1--6},
  year={2017},
  organization={IEEE}
}

@article{kuhn1955hungarian,
  title={{The Hungarian method for the assignment problem}},
  author={{Kuhn, Harold W}},
  journal={{Naval research logistics quarterly}},
  NOvolume={2},
  NOnumber={1-2},
  NOpages={83--97},
  year={1955}
}

@article{barrick1973fmcw,
  title={{FM/CW radar signals and digital processing}},
  author={{Barrick, Donald E}},
  journal={{Report AD-774 829, NOAA}},
  NONOaddress={Boulder, Colorado, USA},
  month={Jul},
  year={1973}
}

@article{willen2013walking,
  title={{Walking speed indoors and outdoors in healthy persons and in persons with late effects of polio}},
  author={Willen, Carin and Lehmann, Kirsten and Sunnerhagen, Katharina},
  journal={Journal of Neurology Research},
  volume={3},
  NOnumber={2},
  NOpages={62--67},
month={Apr},
  year={2013}
}

@article{gennarelli2015multiple,
  title={Multiple extended target tracking for through-wall radars},
  author={Gennarelli, Gianluca and Vivone, Gemine and Braca, Paolo and Soldovieri, Francesco and Amin, Moeness G},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={53},
  NOnumber={12},
  NOpages={6482--6494},
month={Dec},
  year={2015},
  publisher={IEEE}
}

@inproceedings{fitzgerald1986development,
  title={{Development of practical PDA logic for multitarget tracking by microprocessor}},
  author={Fitzgerald, Robert J},
  booktitle={American Control Conference},
NOaddress={Seattle, Washington, USA},
month={Jun},
  year={1986}
}

@article{koch2008bayesian,
  title={Bayesian approach to extended object and cluster tracking using random matrices},
  author={Koch, Johann Wolfgang},
  journal=IEEE_J_AES,
  volume={44},
  NOnumber={3},
  NOpages={1042--1059},
month={Oct},
  year={2008},
}

@article{granstrom2017extended,
	title={{Extended Object Tracking: Introduction, Overview, and Applications}},
	author={Granstr{\"o}m, Karl and Baum, Marcus and Reuter, Stephan},
	journal={Journal of Advances in Information Fusion},
	volume={12},
	NOnumber={2},
	month={Feb},
	year={2017}
}


@article{feldmann2010tracking,
  title={{Tracking of extended objects and group targets using random matrices}},
  author={Feldmann, Michael and Franken, Dietrich and Koch, Wolfgang},
  journal={IEEE Transactions on Signal Processing},
  volume={59},
  NOnumber={4},
  NOpages={1409--1420},
month={Dec},
  year={2010}
}

@inproceedings{rocha2002image,
  title={{Image moments-based structuring and tracking of objects}},
  author={Rocha, Lourena and Velho, Luiz and Carvalho, Paulo Cezar Pinto},
  booktitle={XV Brazilian Symposium on Computer Graphics and Image Processing},
NOaddress={Fortaleza, Brazil},
month={Oct},
  year={2002}
}

@article{zunic2000efficiency,
  title={Efficiency of characterizing ellipses and ellipsoids by discrete moments},
  author={Zunic, Jovisa and Sladoje, Natasa},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={22},
  NOnumber={4},
  NOpages={407--414},
month={Apr},
  year={2000}
}

@article{gennarelli2015multiple,
  title={Multiple extended target tracking for through-wall radars},
  author={Gennarelli, Gianluca and Vivone, Gemine and Braca, Paolo and Soldovieri, Francesco and Amin, Moeness G},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={53},
  NOnumber={12},
  NOpages={6482--6494},
month={Jun},
  year={2015}
}

@inproceedings{meng2020gait,
  title={{Gait Recognition for Co-Existing Multiple People Using Millimeter Wave Sensing}},
  author={Meng, Zhen and others},
  booktitle={Proc.~AAAI},
NOaddress={New York, New York, USA},
month={Feb},
  year={2020}
}


@article{bordonaro2014decorrelated,
	title={{Decorrelated unbiased converted measurement Kalman filter}},
	author={Bordonaro, Steven and Willett, Peter and Bar-Shalom, Yaakov},
	journal=IEEE_J_AES,
	volume={50},
	NOnumber={2},
	NOpages={1431--1444},
	month={Jul},
	year={2014}
}


@article{pegoraro2020multiperson,
	title={{Multi-Person Continuous Tracking and Identification from mm-Wave micro-Doppler Signatures}},
	author={Pegoraro, Jacopo  and Meneghello, Francesca and Rossi, Michele},
	journal={IEEE Transactions on Geoscience and Remote Sensing},
	volume={59},
	NOnumber={4},
	NOpages={2994 - 3009},
	month={Apr},
	year={2021},
	doi={10.1109/TGRS.2020.3019915}
}

@book{richards2010principles,
	title={Principles of modern radar},
	author={Richards, Mark A and Scheer, Jim and Holm, William A and Melvin, William L},
	publisher={Scitech Publishing Inc.},
	NOaddress={Raleigh, NC, USA},
	year={2010}
}

@article{vaishnav2020continuous,
	title={{Continuous Human Activity Classification With Unscented Kalman Filter Tracking Using FMCW Radar}},
	author={Vaishnav, Prachi and Santra, Avik},
	journal={IEEE Sensors Lett.},
	NOvolume={4},
	NOnumber={5},
	NOpages={1--4},
	month={Apr},
	year={2020}
}

@article{lerro1993tracking,
	title={{Tracking with debiased consistent converted measurements versus EKF}},
	author={Lerro, Don and Bar-Shalom, Yaakov},
	journal=IEEE_J_AES,
	volume={29},
	NOnumber={3},
	NOpages={1015--1022},
	month={Jul},
	year={1993}
}

@book{benvenuto2021algorithms,
	title={Algorithms for communications systems and their applications},
	author={Benvenuto, Nevio and Cherubini, Giovanni and Tomasin, Stefano},
	year={2021},
	publisher={John Wiley \& Sons}
}

@book{bishop2006pattern,
	title={Pattern recognition and machine learning},
	author={Bishop, Christopher M},
	year={2006},
	publisher={Springer}
}

@inproceedings{feng2020evaluating,
	title={{Evaluating mmWave Sensing Ability of Recognizing Multi-people Under Practical Scenarios}},
	author={Feng, Lipeng and Du, Shibo and Meng, Zhen and Zhou, Anfu and Ma, Huadong},
	booktitle={International Conference on Green, Pervasive, and Cloud Computing},
	NOpages={61--74},
	month={Dec},
	year={2020},
	organization={Springer}
}


@book{simon2006optimal,
	title={{Optimal state estimation: Kalman, H infinity, and nonlinear approaches}},
	author={Simon, Dan},
	year={2006},
	publisher={John Wiley \& Sons}
}

@book{nocedal2006numerical,
	title={Numerical optimization},
	author={Nocedal, Jorge and Wright, Stephen},
	year={2006},
	publisher={Springer Science \& Business Media}
}

@article{cheng2021person,
  title={Person Reidentification Based on Automotive Radar Point Clouds},
  author={Cheng, Yuwei and Liu, Yimin},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  month={Early Access},
  year={2021},
  publisher={IEEE}
}


@article{pegoraro2021real,
  title={Real-time People Tracking and Identification from Sparse mm-Wave Radar Point-clouds},
  author={Pegoraro, Jacopo and Rossi, Michele},
  journal={IEEE Access},
  NOvolume={9},
  NOpages={ 78504 - 78520},
  month={May},
  year={2021},
  publisher={IEEE}
}

@article{shalom2009probabilistic,
  author={Bar-Shalom, Yaakov and Daum, Fred and Huang, Jim},
  journal={IEEE Control Syst. Mag.}, 
  title={The probabilistic data association filter}, 
  year={2009},
  volume={29},
  NOnumber={6},
  NOpages={82-100}}
  
@article{ribeiro2004kalman,
  title={Kalman and extended kalman filters: Concept, derivation and properties},
  author={Ribeiro, Maria Isabel},
  journal={Institute for Systems and Robotics},
  volume={43},
  NOpages={46},
  year={2004},
  publisher={Citeseer}
}

@inproceedings{silbert2014new,
  title={New metrics for quantifying data association performance},
  author={Silbert, Mark E and Agate, Craig S},
  booktitle={Proc~IEEE FUSION},
  NOpages={1--8},
  year={2014},
  NOorganization={IEEE}
}

@inproceedings{guendel2021continuous,
  title={Continuous human activity recognition for arbitrary directions with distributed radars},
  author={Guendel, Ronny Gerhard and others},
  booktitle={Proc.~IEEE RadarConf21},
  NOaddress={Atlanta, GA, USA},
  month={May},
  year={2021}
}

@inproceedings{li2021pedestrian,
  title={Pedestrian Trajectory based Calibration for Multi-Radar Network},
  author={Li, Shuai and others},
  booktitle={Proc.~IEEE INFOCOM WKSHPS},
  NONOaddress={Vancouver, BC, Canada},
  month={May},
  year={2021}
}

@article{iwata2021multiradar,
  title={Multiradar data fusion for respiratory measurement of multiple people},
  author={Iwata, Shunsuke and Koda, Takato and Sakamoto, Takuya},
  journal=IEEE_J_SENSOR,
  volume={21},
  NOnumber={22},
  NOpages={25870--25879},
  month={Oct},
  year={2021},
  publisher={IEEE}
}

@article{sorkine2017least,
  title={Least-squares rigid motion using {SVD}},
  author={Sorkine-Hornung, Olga and Rabinovich, Michael},
  journal={Computing},
  NOvolume={1},
  NOnumber={1},
  NOpages={1--5},
  year={2017}
}

@article{chang1997optimal,
  title={On optimal track-to-track fusion},
  author={Chang, Kuo-Chu and Saha, Rajat K and Bar-Shalom, Yaakov},
  journal=IEEE_J_AES,
  volume={33},
  NOnumber={4},
  NOpages={1271--1276},
  month={Oct},
  year={1997},
  publisher={IEEE}
}

@article{chong2000architectures,
  title={Architectures and algorithms for track association and fusion},
  author={Chong, Chee-Yee and Mori, Shozo and Barker, William H and Chang, Kuo-Chu},
  journal=IEEE_M_AES,
  volume={15},
  NOnumber={1},
  NOpages={5--13},
  month={Jan},
  year={2000},
  NOpublisher={IEEE}
}


@ARTICLE{steiner2020millimeter,
  author={Steiner, Maximilian and Grebner, Timo and Waldschmidt, Christian},
  journal={IEEE Trans. Microw. Theory Techn.}, 
  title={{Millimeter-Wave SAR-Imaging With Radar Networks Based on Radar Self-Localization}}, 
  month={Nov},
  year={2020},
  volume={68},
  NOnumber={11},
  NOpages={4652-4661},
  doi={10.1109/TMTT.2020.2995225}}
  
@INPROCEEDINGS{xu2019millimeter,
  author={Xu, Yi and others},
  booktitle={Proc.~IEEE SmartWorld},
  title={Millimeter-Wave Multi-Radar System for Ubiquitous Concealed Dangerous Object Detection}, 
  year={2019},
  volume={},
  number={},
month = {Aug},
  doi={10.1109/SmartWorld-UIC-ATC-SCALCOM-IOP-SCI.2019.00333}}

@article{javadi2020radar,
  title={Radar networks: A review of features and challenges},
  author={Javadi, S Hamed and Farina, Alfonso},
  journal={Information fusion},
  volume={61},
  NOpages={48--55},
  month={Sept},
  year={2020},
  publisher={Elsevier}
}

@article{folster2005data,
  title={Data association and tracking for automotive radar networks},
  author={Folster, Florian and Rohling, Hermann},
  journal=IEEE_J_ITS,
  volume={6},
  NOnumber={4},
  NOpages={370--377},
  month={Dec},
  year={2005},
  publisher={IEEE}
}

@article{geng2020evolution,
  title={Evolution of netted radar systems},
  author={Geng, Zhe},
  journal={IEEE Access},
  volume={8},
  NOpages={124961--124977},
  month={Jul},
  year={2020},
  publisher={IEEE}
}

@inproceedings{shu2007data,
  title={Data fusion in a multi-target radar sensor network},
  author={Shu, Haining and Liang, Qilian},
  booktitle={Proc.~IEEE RWS},
  address={Long Beach, CA, USA},
  month={Jan},
  year={2007},
  NOorganization={IEEE}
}

@article{ledergerber2020multi,
  title={A multi-static radar network with ultra-wideband radio-equipped devices},
  author={Ledergerber, Anton and D’Andrea, Raffaello},
  journal={Sensors},
  volume={20},
  NOnumber={6},
  NOpages={1599},
  month={Mar},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{cowley1993registration,
  title={Registration in multi-sensor data fusion and tracking},
  author={Cowley, Derek C and Shafai, Bahram},
  booktitle={1993 American Control Conference},
  NOpages={875--879},
  month={Jun},
  address={Sen Francisco, CA, USA},
  year={1993},
  organization={IEEE}
}

@inproceedings{wang2021distributed,
  title={Distributed Registration and Multi-target Tracking with Unknown Sensor Fields of View},
  author={Wang, Ziting and others},
  booktitle={2021 IEEE Radar Conference (RadarConf21)},
address={Atlanta, GA, USA},
month={May},
address={Heidelberg, Germany},
  year={2021},
  organization={IEEE}
}

@inproceedings{uney2016distributed,
  title={Distributed localisation of sensors with partially overlapping field-of-views in fusion networks},
  author={{\"U}ney, Murat and Mulgrew, Bernard and Clark, Daniel},
  booktitle={2016 19th International Conference on Information Fusion (FUSION)},
month={Jul},
  year={2016},
  organization={IEEE}
}

@inproceedings{bernardin2006multiple,
  title={Multiple object tracking performance metrics and evaluation in a smart room environment},
  author={Bernardin, Keni and Elbs, Alexander and Stiefelhagen, Rainer},
  booktitle={Proc.~IEEE Int. Wkshp. on Vis. Surveillance},
  volume={90},
  NOnumber={91},
  year={2006},
  NOorganization={Citeseer}
}

@ARTICLE{canil2022-milliTRACE-IR,
  author={Canil, Marco and Pegoraro, Jacopo and Rossi, Michele},
  journal=IEEE_J_STSP, 
  title={{milliTRACE-IR: Contact Tracing and Temperature Screening via mmWave and Infrared Sensing}}, 
  year={2022},
  volume={16},
  NOnumber={2},
  NOpages={208-223},
  doi={10.1109/JSTSP.2021.3138632}}
